A Sublinear Algorithm for Sparse Reconstruction with l2/l2 Recovery Guarantees

Compressed Sensing aims to capture attributes of a sparse signal using very few measurements. Cand\`{e}s and Tao showed that sparse reconstruction is possible if the sensing matrix acts as a near isometry on all $\boldsymbol{k}$-sparse signals. This property holds with overwhelming probability if the entries of the matrix are generated by an iid Gaussian or Bernoulli process. There has been significant recent interest in an alternative signal processing framework; exploiting deterministic sensing matrices that with overwhelming probability act as a near isometry on $\boldsymbol{k}$-sparse vectors with uniformly random support, a geometric condition that is called the Statistical Restricted Isometry Property or StRIP. This paper considers a family of deterministic sensing matrices satisfying the StRIP that are based on \srm codes (binary chirps) and a $\boldsymbol{k}$-sparse reconstruction algorithm with sublinear complexity. In the presence of stochastic noise in the data domain, this paper derives bounds on the $\boldsymbol{\ell_2}$ accuracy of approximation in terms of the $\boldsymbol{\ell_2}$ norm of the measurement noise and the accuracy of the best $\boldsymbol{k}$-sparse approximation, also measured in the $\boldsymbol{\ell_2}$ norm. This type of $\boldsymbol{\ell_2 /\ell_2}$ bound is tighter than the standard $\boldsymbol{\ell_2 /\ell_1}$ or $\boldsymbol{\ell_1/ \ell_1}$ bounds.

==> klarge.tex <==
When $k$ is large, at each iteration, Step 8 of the Algorithm~\ref{alg1} requires finding the pseudoinverse of a $\m\times k$ matrix. In this case, we provide a more efficient, and algorithm which requires finding the pseudoinverse of a $1 \times k$ sub-matrix. Algorithm~\ref{alg2} at each iteration only updates one entry of $\has$
Here $\Theta$ is a lookup table. If at some round $t$, the recovered position $p$ has been previously recovered at some previous round $t'$, the we restore the recovered value ${\beta^*}_{t'}$. This allows that instead of recovering a new value ${\beta^*}_{t}$ based on $\yy-{\beta^*}_{t'}\varphi_{P_{p},b_{p}}$, and then outputting  ${\beta^*}_{t}+{\beta^*}_{t'}$, we can output a more precise value ${\beta^*}_{t}$ based on $\yy$.
 \begin{algorithm}[h]
\caption{Faster Quadratic Decoding Algorithm}
   Input: $\m$ dimensional vector $\boldsymbol{f}=\A \bs{\alpha}+\nu$\\
   Output: An approximation $\bs{\beta^k}$ to the signal $\bs{\alpha}$\\
     \label{alg2}
   \begin{algorithmic}[1]
   \STATE Set $\yy_1=\yy$, $\Theta=\{\}$.
   \FOR{$t=1,\cdots,k$ or while $\|\boldsymbol{f_t}\|_2 \geq \epsilon$}
   \FOR{ each entry $x=1$ to $\m$}\label{a1}
   \STATE pointwise multiply $\yy_t$ with a shift (offset) of itself as in~(\ref{walsh}).
   \ENDFOR 
   \STATE Compute the fast Walsh-Hadamard transform of the pointwise product: Equation~(\ref{fourier}) \label{a2}
   \STATE Find the position of the next peak $\boldsymbol{e}_{p_t}$ in the Hadamard domain: Equation~(\ref{chirp}) implies that the chirp-like cross terms appear as a constant background signal. \label{a3}
   \IF{$p_t \in \mbox{Keys}(\Theta)$} \label{a4}
   \STATE Restore $\boldsymbol{f_t}\leftarrow \boldsymbol{f_t}+\Theta(p_t) \varphi_{P_{p_t},b_{p_t}}$.
   \ENDIF
   \STATE  \label{opt2} Update  $\bs{\beta^t}\doteq \yy^\top \varphi_{P_{p_t},b_{p_t}} $ which minimizes $\|\boldsymbol{f_t}-\beta_t \varphi_{P_{p_t},b_{p_t}}\|_2$. (StRIP property) 
   \STATE Set $\has^{t+1}\leftarrow \has^t+ \beta_t \boldsymbol{e}_{p_t}.$
   \STATE Set $\Theta(p_t)= \beta_t.$
   \STATE Set $\boldsymbol{f_{t+1}}\leftarrow \boldsymbol{f_t}- \beta_t \varphi_{P_{p_t},b_{pi_t}}$. \label{a5}
   \ENDFOR
   \end{algorithmic}
   \end{algorithm}

\begin{rem}Note that  Step~\ref{opt} of Algorithm~\ref{alg2} is a normal regression task and has analytical solution
\begin{equation}
\bs{\beta^t}\doteq\left( \lng^\top{\overline{\lng}}\right)^{-1} \lng^\top f=\lng^\top \yy,
\end{equation}
the second equality is based on the uni-modularity of the entries of $\A$. \end{rem}
\begin{rem}
Step \ref{a1} takes $O(\m)$ computation time. Computing the Hadamard transform takes $\m \log^\m$ time. Steps \ref{a3}, \ref{a4}, \ref{opt2}, \ref{a5} all take $O(\m)$ time to compute. Hence, the total time complexity of the algorithm~\ref{alg2}, is $k\m \log^2 \m$.
\end{rem}


==> matback.tex <==
Let $m$ be an odd integer, the rows of the sensing matrix $\A$ are indexed by binary $m$-tuples $x$, and the columns are indexed by pairs $P,b$, where $P$ is an $m\times m$ binary symmetric matrix and $b$ is a binary $m$-tuple. The entry $\varphi_{P,b}(x)$ is given by 
\begin{equation}
\label{kerdock}
\varphi_{P,b}(x)=i^{wt(d_P)+2wt(b)}i^{x^\top Px+2b^\top x}
\end{equation}
where $d_p$ denotes the main diagonal of $P$. Note that all arithmetic in the exponent $xPx^\top+2bx^\top$ takes place in the ring of integers modulo $4$. If we fix a matrix $P$, then the $2^m$ columns $\varphi_{P,b}~,~b\in \mathbb{F}_2^m$ form an orthonormal basis $\Gamma_P$ that is obtained by postmultiplying the Walsh-Hadamard basis by the unitary transformation $\mbox{diag}\left[ i^{xPx^\top}\right]$.

\begin{lemma}
\label{l1}
The diagonal $d_P$ of a binary symmetric matrix $P$ is contained in the row space of $P$.
\end{lemma}
\begin{proof}
We suppose that there is no solution to the equation $zP=d_P$ and show that the vector $\left[ i^{xPx^\top}\right]$ is diagonal to every vector in the Walsh-Hadamard orthonormal basis. Set
$$S=\left( \left( i^{xPx^\top}\right),\left( i^{2bz^\top}\right) \right)=\sum_x i^{x^\top Px+2b^\top x}. $$
Then
\begin{eqnarray}
\nonumber S^2&=& \sum_{x,y}  i^{x^\top Px+y^\top Py+2b(x+y)^\top}
\\ \nonumber &=& \sum_{x,y}  i^{(x+y)^\top P(x+y)+2xPy^\top +2b(x+y)^\top}.
\end{eqnarray}
Changing the variables $z=x\oplus y$ and $y$ gives
$$ S^2=\sum_z  i^{zPz^\top} \sum_y (-1)^{(d_P+zP)y^\top},$$
and since there is no solution to $zP=d_P$, we have $S=0$.
\end{proof}
\begin{lemma}
If $S=\sum_x i^{x^\top Px+2b^\top x}$, then either $S=0$ or 
$$S^2=\sum_{z_1}  i^{z_1Pz^\top_1+2bz^\top_1}2^{2m-R},$$ where $z_1 P=d_P$ and $R$ is the rank of the binary symmetric matrix $P$.
\end{lemma}
\begin{proof}As in the proof of the Lemma~\ref{l1}
$$ S^2=\sum_z  i^{zPz^\top} \sum_y (-1)^{(d_P+zP)y^\top}.$$
The solutions to the Equation $zP=0$ form a vector space $E$ and for all $e,f\in E,$
$$ePe^\top+fPf^\top=(e+f)P(e+f)^\top~~(\mbox{mod}~4~).$$
Hence
\begin{eqnarray}
\nonumber S^2&=& 2^m\sum_{e\in E}  i^{(z_1+e)P(z_1+e)^\top+2b(z_1+e)^\top}
\\ \nonumber &=& 2^m i^{z_1Pz^\top_1+2z^\top_1b}\sum_{e \in E}  i^{ePe^\top+2be^\top}.
\end{eqnarray}
The map $e\rightarrow ePe^\top$ is a linear map from $E$ to $\mathbb{Z}_2$ so that the numerator $ePe^\top+2be^\top$ also defines a linear map from $E$ to $\mathbb{Z}_2$. If this linear map is the zero map then 
$$S^2=2^{2m-R}  i^{z_1Pz^\top_1+2bz^\top_1},$$ and if it is nonzero then $S=0$.

\end{proof}


